Neutron Skins: Weak Elastic Scattering and Neutron Stars

The recently completed PREX-2 campaign - which measured the weak form factor of lead at an optimal momentum transfer - has confirmed that the neutron skin of lead is relatively large and has provided a precise determination of the interior baryon density of a heavy nucleus. In turn, the measured form factor can be related to various nuclear and neutron-star properties. Astrophysical observations by the NICER mission have benefited from improvements in flux, energy resolution, and notably, timing resolution. NICER has the capability to measure pulse profile data, which enables simultaneous mass-radius determinations. During the next decade, measurements in astrophysics, gravitational wave astronomy, and nuclear physics are expected to provide a wealth of more precise data. In this review we provide an overview of the current state of neutron skin measurements and offer insights into the prospects for the future.

==> notes.tex <==
\section{Main papers reviewed [notes for us, not to be included except possibly as references]}
\begin{itemize}
    \item 
Precision Determination of the Neutral Weak Form Factor of 48Ca, D. Adhikari et al, ArXiv:2205.11593, Phys. Rev. Lett. 129, 042501  (2022)
\item
First Determination of the 27Al Neutron Distribution Radius from a Parity-Violating Electron Scattering Measurement, Qweak collaboration, arXiv:2112.15412, Phys. Rev. Lett. 128, 132501 (2022)
\item
 Implications of PREX-II on the equation of state of neutron-rich matter, Brendan T. Reed, F. J. Fattoyev, C. J. Horowitz, Jorge Piekarewicz,  PRL 126, 172503 (2021) 
\item
An Accurate Determination of the Neutron Skin Thickness of 208Pb through Parity-Violation in Electron Scattering, KK, Paul Sauder, Kent Pasckke, Ciprian Gal … PRL 126, 172502 (2021)

\item
 Measuring the surface thickness of the weak charge density of nuclei, Brendan R. Reed, Z. Jaffe, C. J. Horowitz and C. Sfienti, Phys. Rev. C 102, 064308 (2020).

 \item
 Insights into nuclear saturation density from parity violating electron scattering, C. J. Horowitz, J. Piekarewicz, and Brendan Reed, Phys. Rev. C 102 (2020) 044321

 \item
 Neutron skins of atomic nuclei: per aspera ad astra, M. Thiel , C. Sfienti, J. Piekarewicz, C. J. Horowitz, and M. Vanderhagen, Topical Review, M Thiel et al 2019 J. Phys. G: Nucl. Part. Phys. 46 093003

 \item
 Neutron skins and neutron stars in the multi-messenger era, F. J. Fattoyev, J. Piekarewicz, and C. J. Horowitz, Phys. Rev. Lett. 120, 172702 (2018) 

 
\item  B. Hu et al., Nature Phys. 18, 1196 (2022).https://www.nature.com/articles/s41567-022-01715-8
\itemP.-G. Reinhard, X. Roca-Maza, and W. Nazarewicz,
(2022), arXiv:2206.03134 [nucl-th].
\itemZ. Zhang and L.-W. Chen, (2022), arXiv:2207.03328
[nucl-th].
\itemC. Mondal and F. Gulminelli, (2022), arXiv:2209.05177
[nucl-th].
\itemP. Papakonstantinou (2022) arXiv:2210.02696 [nucl-th].
\item E. Y ̈uksel and N. Paar, Phys. Lett. B 836, 137622 (2023),
arXiv:2206.06527 [nucl-th].

\end{itemize}

%Disclosure
